PAC-Bayesian Learning of Aggregated Binary Activated Neural Networks with Probabilities over Representations

Considering a probability distribution over parameters is known as an efficient strategy to learn a neural network with non-differentiable activation functions. We study the expectation of a probabilistic neural network as a predictor by itself, focusing on the aggregation of binary activated neural networks with normal distributions over real-valued weights. Our work leverages a recent analysis derived from the PAC-Bayesian framework that derives tight generalization bounds and learning procedures for the expected output value of such an aggregation, which is given by an analytical expression. While the combinatorial nature of the latter has been circumvented by approximations in previous works, we show that the exact computation remains tractable for deep but narrow neural networks, thanks to a dynamic programming approach. This leads us to a peculiar bound minimization learning algorithm for binary activated neural networks, where the forward pass propagates probabilities over representations instead of activation values. A stochastic counterpart that scales to wide architectures is proposed.

==> figures/stochastic_abnet.tex <==
\tikzset{%
	every neuron/.style={
		circle,
		draw,
		minimum size=0.2cm
	},
	neuron missing/.style={
		circle,
		draw=lightgray,
		minimum size=0.2cm
	},
	neuron missingdots/.style={
		draw=none, 
		scale=2,
		text height=0.3cm,
		execute at begin node=\color{black}$\vdots$
	}
}

\begin{tikzpicture}[x=0.8cm, y=0.8cm, >=stealth]
	
	% defining nodes
	
	\foreach \m [count=\y] in {1,2,3,4}
	\node [every neuron] (data-\m) at (0,9.5-2*\y) {};
	
	\foreach \m [count=\y] in {missing,1,missing,2,missing,missing,3,missing}
	\node [every neuron/.try, neuron \m/.try] (input-\m) at (2,9-\y) {};
	
	\foreach \m [count=\y] in {missing,1,missing,missing,missing,missing,2,missing,missingdots,3}
	\node [every neuron/.try, neuron \m/.try] (hidden1-\m) at (4,10-\y) {};
	
	\foreach \m [count=\y] in {1,2,missing,3}
	\node [every neuron/.try, neuron \m/.try] (hidden2-\m) at (6,9.5-2*\y) {};	
	
	\foreach \m [count=\y] in {1}
	\node [every neuron] (output-\m) at (8,4.5) {};
	
	%defining connections
	
	\foreach \i in {1,...,4}
	\foreach \j in {1,...,3}
	\draw [->] (data-\i) -- (input-\j);
	
	\foreach \i in {1,...,3}
	\foreach \j in {1,...,3}
	\draw [->] (input-\i) -- (hidden1-\j);
	
	\foreach \i in {1,...,3}
	\foreach \j in {1,...,3}
	\draw [->] (hidden1-\i) -- (hidden2-\j);
	
	\foreach \i in {1,...,3}
	\foreach \j in {1,...,1}
	\draw [->] (hidden2-\i) -- (output-\j);
	
	\foreach \l [count=\i] in {1}
	\draw [->] (output-\i) -- ++(1,0)
	node [above, midway] {};
	
\end{tikzpicture}

==> figures/stochastic_compact_abnet.tex <==
\tikzset{%
	every neuron/.style={
		circle,
		draw,
		minimum size=0.2cm
	},
	neuron missing/.style={
		circle,
		draw=lightgray,
		minimum size=0.2cm
	}
}

\begin{tikzpicture}[x=0.8cm, y=0.8cm, >=stealth]
	
	% defining nodes
	
	\foreach \m [count=\y] in {1,2,3,4}
	\node [every neuron] (data-\m) at (0,9.5-2*\y) {};
	
	\foreach \m [count=\y] in {missing,1,missing,2,missing,missing,3,missing}
	\node [every neuron/.try, neuron \m/.try] (input-\m) at (2,9-\y) {};

	\foreach \m [count=\y] in {1}
	\node [every neuron] (output-\m) at (8,4.5) {};
	
	%defining connections
	
	\foreach \i in {1,...,4}
	\foreach \j in {1,...,3}
	\draw [->] (data-\i) -- (input-\j);
	
	\foreach \i in {1,...,3}
	\foreach \j in {1,...,1}
	\draw [->] (input-\i) -- (output-\j);
	
	\foreach \l [count=\i] in {1}
	\draw [->] (output-\i) -- ++(1,0)
	node [above, midway] {};
	
\end{tikzpicture}


==> sections/rebuttal.tex <==

\textbf{Rebuttal distillation : what to include / put the emphasis on}\\
%\textbf{1} Mettre l'emphase sur ($\star$) et ($\star\star$)\\
%$\checkmark$ Mettre l'accent sur les nouveautés de l'article par rapport à PBGNet / les contributions originales: the compact scheme and the analysis of the dichotomy between the first layers versus the others are new (mentionné dans la conclusion, pas vraiment dans l'abstract/intro)\\
%$\checkmark$ Mettre l'emphase sur le fait que les approximations de PBGNet et ABNet sont différentes\\
%$\checkmark$ How the number of hidden layers is chosen for each model? Our experiments focus on the ability to perform accurate model selection. In Table 1, PBGNet and ABNet lines display the models with the lowest PAC-Bayes bounds. Others (PBGNetl, ABNetl and EBP) display the models with the best validation score. We will definitely clarify this.\\
Commentaires quant au travail de Biggs et Guedj: "Differentiable PAC-Bayes objectives with partially aggregated neural networks"\\
%$\checkmark$ Connections with NNGP ("Deep neural networks as gaussian processes") and NTK ("Neural tangent kernel: Convergence and generalization in neural networks"). Although implying a distribution over weights, these (major) works study the convergence of infinitely wide networks, while we deliberately focus on finite and discrete models as our building blocks. We will mention that PAC-Bayes allows obtaining generalization bounds in the finite regime, and cite NNGP and NTK papers as seminal approaches leveraging other probabilistic views of neural networks\\
